Performance-oriented DevOps: A Research Agenda

DevOps is a trend towards a tighter integration between development (Dev) and operations (Ops) teams. The need for such an integration is driven by the requirement to continuously adapt enterprise applications (EAs) to changes in the business environment. As of today, DevOps concepts have been primarily introduced to ensure a constant flow of features and bug fixes into new releases from a functional perspective. In order to integrate a non-functional perspective into these DevOps concepts this report focuses on tools, activities, and processes to ensure one of the most important quality attributes of a software system, namely performance. Performance describes system properties concerning its timeliness and use of resources. Common metrics are response time, throughput, and resource utilization. Performance goals for EAs are typically defined by setting upper and/or lower bounds for these metrics and specific business transactions. In order to ensure that such performance goals can be met, several activities are required during development and operation of these systems as well as during the transition from Dev to Ops. Activities during development are typically summarized by the term Software Performance Engineering (SPE), whereas activities during operations are called Application Performance Management (APM). SPE and APM were historically tackled independently from each other, but the newly emerging DevOps concepts require and enable a tighter integration between both activity streams. This report presents existing solutions to support this integration as well as open research challenges in this area.

==> 2.4-Performance_Problems.tex <==
\subsection{APM-Tooling Theory \& Practice}
\label{sec:performanceProblems}

APM-Tooling Theory \& Practice


==> 4.2-Extraction_of_Load_Intesity_and_Navigational_Profiles.tex <==
\subsection{Workload Classification and Forecasting}
% \label{sec:extractionLoadIntensity}
% 
% -> Telco with Andre 26.1.: Extraction of Load Intensity and Navigational
% Profiles fits better in the model extraction chapter: 2.3.2  and is now covered
% there.
% 
% Proposal for new content: Rename Chapter 4.2
% to something like ``Forecasting and Anomaly Detection at System Run-Time''
% 
% -> Run-Time aspects: Model Calibration, Forecasting using Time Series Analysis
% and Models, Anomaly metrics, Dynamic System reconfigurations (e.g. resource
% provisioning and migration in elastic IaaS clouds?). 
% 
% --> Should we open this new topic and keep it just short. Or better include it
% as an paragraph in APM section (as already covered in the notes of this
% section) - and model-calibration in 4.3.
% 
% =============
% 
% covered in section 2.3.2:
% Load profiles (seasonal, trends, noise, burst)\\
% (High-Level) Descartes Load Intensity Model\\
% Automatic extraction of load intensity profiles\\
% Markov4JMeter, Behavior models\\
% User group clustering\\
% 
% \cite{kistowski2014} \cite{kistowski2014a} \cite{kistowski2014b}
% \todo{Only include problem diagnosis and detection based on monitoring data}

\todo{Would be nice to have \ldots}

==> Model-Driven_Performance_Measurement.tex <==
\subsection{Model-Driven Performance Measurement}
\label{sec:modelDrivenPerformanceMeasurement}

Model-driven software engineering (MDE) utilizes models for many different views and aspects of software systems. These models are then used to automatically generate most of the programming code, configuration setups, and other artifacts required to implement a software system.

One key aspect of software systems is their observation at run-time to be evaluate performance qualities. While with present monitoring framework this task is highly technology dependent which results in different specific solutions for each technology. For example, Kieker \citep{vanhoorn2014dynamic} supports various languages including C, Perl and Java. For each language and each framework implemented in those languages separate probes and samplers have been implemented and must be configured and setup separately.  
% what are the goals of model driven measurements?
% - Abstraction from concrete probe/sensor technology
% - Abstraction form concrete introduction technology, languages etc.
% - Providing a consistent and standardizied view on speciying measures
The goal of model-driven measurements is the abstraction from such technological details and providing an abstract notation for all probes and samplers. This improves the compatibility and comparability of measurements and eases the specification of monitoring. Furthermore, such models could be used to be integrated in an MDE approach to define the placement of probes and samplers on the basis of architectural models.

% what is required?
%   - run time support and frameworks
%   - mapping or interpreting instrumentation join points
As with every model-driven approach, the abstraction requires run time support in form of a run time library and framework, as well as a transformation to realize the necessary implementation level configuration and code artifacts or an interpreter of the instrumentation model to realize the weaving of monitoring aspect and application.

% Solutions: What do they cover in general
% - IAL/IRL - Jung
% - MoDePemArt - Boscovik
% - AIM - Wert
Model-driven monitoring is a relatively new research topic starting with research of \citet{Boskovic2006,Boskovic2009} which targets information systems and two recent approaches one with an MDE background \citep{Jung2013} introducing two languages to model observation data, probes, and probe placements and one developed initially for application testing \citep{Wert2015}, called AIM.

% discrimination from
% - SPASSMeter manual code modification
% - Kieker instrumentation with 
%   - AspectJ for application code
%   - Interceptors, Listeners in Java EE
% - All very technology dependent no uniform approach to application and system
%   monitoring no abstraction from implementation technologies


% Explain AIM
\subsubsection{Adaptable Instrumentation and Monitoring} 
% - Focus measuring applications under test
% - Provides an abstraction for instrumentation in
%   - Application level probes
%   - Hardware and OS sampling
% - Coverage
%   - hw, os and application level
% - Features
%   - Extensible
%   - Include monitoring framework
The origin of AIM is observing applications under test (AUT). It comprises a run time byte code weaving capability to realize adaptive monitoring with less overhead on the application execution compared to frameworks, like Kieker, which 
realize adaptive monitoring by integrating an additional conditional statement, resulting in an performance impact even when the probe is inactive. On top of this run time byte code weaving approach, AIM provides a meta-model to describe probe placement and sampler configuration which is divided in defining a scope for the probes and adding restriction based on the package structure. At present AIM supports samplers different hardware and operating system sources, like CPU, disk, network, and memory, and probes, like response time, traces, and memory footprint. Furthermore, AIM is designed to be extended with additional probes and samples. By that AIM covers hardware, operating system and application level
monitoring. However, at present AIM is bound to Java, as is visible through the package based restrictions. Even though other languages have similar concepts, like name spaces, the package concept less flexible. Furthermore, AIM defines placements based on programming code and not an abstract application model covering the architecture.
  
% Explain ModePemart
\subsubsection{Model Driven Performance Measurement and Assessment}
% - Focus
%   - UML
%   - runtime observation of deployed application
% - Abstraction
%   - Abstraction on UML model level
%   - Measurement point/join point, metric and context
% - Coverage
%   - Transformational and Reactive systems
%   - Measurement and assessment
Model Driven Performance Measurement and Assessment with Relational Traces (MoDePeMART) is an approach for instrumenting and monitoring informations systems, and encompasses observation and assessment of such systems \citep{Boskovic2009}. It is rooted in the UML modeling domain and expresses join points by referencing UML model elements.

% - Features
%   - DSML used to describe monitoring
%   - Integration into the code generation process (theoretically)
%   - Data und monitoring modeling
%   - provides no tooling?
MoDePeMART defines a specific modeling language for monitoring which allows to define monitoring points and measurement evaluations for these points, covering not only monitoring but also the analysis domain. The data model and the realization of the data storage is also part of the approach. However, the integration of monitoring into the code is part of the code generator and not realized explicitly by MoDePeMART. 

% Explain IAL/IRL?
\subsubsection{Instrumentation Record and Aspect Languages}
% - Focus
%   - observation at run time
%   - cloud 
% - Abstraction
%   - Technology and language abstraction
% - Coverage
%   - primary application level
%   - support for other areas depends on extend of modeling
%   - Allows to model new probes in an abstract manner
%   - part of the iObserve approach for model-driven and model-based evaluation
% - Features
%   - Generic/can integrate different monitoring frameworks
%   - Extensible
%   - MDE
%   - data and monitoring modeling
The third approach is part of the iObserve \citep{hasselbring2014} monitoring and analysis framework and rooted in model-driven engineering utilizing on aspect-oriented modeling. It provides a programming language independent data modeling for the monitoring through the instrumentation record language (IRL), technology independent probe specification and meta-model and weaving technology independent point cut notation through the instrumentation aspect language (IAL). 

The IAL is meta-model agnostic and can support different architecture description languages and meta-models, such as repository, allocation and deployment meta-models from PCM \citep{becker2009} and Descartes \citep{Kounev2014}. Therefore, it can be used to describe application level monitoring probes as well as samplers, like AIM. However, its focus and tool support is designed for application level monitoring.

As the IAL defines monitoring point cuts at modeling level and due to its generator based approach, it is prepared to be extended to support different run time environments beside Java EE, different weaving technologies such as AspectJ and DISSL, and can incorporate different monitoring frameworks such as Kieker or AIM which are able to provide implementation level realizations for monitoring. In contrast to AIM, the IAL does not cover adaptive monitoring. However, this is considered a run time behavior and must be provided by the underlying frameworks.

MoDePeMART shows that it is helpful to couple an instrumentation method with metric based evaluation and analysis. Through the implementation independent monitoring specification of the IAL such evaluation can be realized across technologies. While in implementation level monitoring metrics relate to implementation artifacts, in model-driven monitoring these metrics are defined on basis of the application model. However, monitoring technologies such as Kieker and AIM provide only implementation level information. In iObserve, this divide between model and code is bridged by utilizing a trace model relying model elements and abstractions to code elements. This model is first used to map model level point cuts to the implementation level and then later to map implementation level monitoring data back to the modeling level.

All three approaches represent a different view on the subject of model-driven monitoring. Especially AIM, providing already a model-based point cut notation is suited to be combined with IAL and IRL. MoDePeMART provides insights into the combination of monitoring and analysis and the necessity to model monitoring data in an abstract way to be able to support different technologies and platforms.


